An Arduino based heartbeat detection device (ArdMob-ECG) for real-time ECG analysis

This technical paper provides a tutorial to build a low-cost (10-100 USD) and easy to assemble ECG device (ArdMob-ECG) that can be easily used for a variety of different scientific studies. The advantage of this device is that it automatically stores the data and has a built-in detection algorithm for heartbeats. Compared to a clinical ECG, this device entails a serial interface that can send triggers via USB directly to a computer and software (e.g. Unity, Matlab) with minimal delay due to its architecture. Its software and hardware is open-source and publicly available. The performance of the device regarding sensitivity and specificity is comparable to a professional clinical ECG and is assessed in this paper. Due to the open-source software, a variety of different research questions and individual alterations can be adapted using this ECG. The code as well as the circuit is publicly available and accessible for everyone to promote a better health system in remote areas, Open Science, and to boost scientific progress and the development of new paradigms that ultimately foster innovation.

==> Deleted_passages.tex <==

\hspace{-0.5cm}Tim Julian Möller\,$^{1,*}$,  Keisuke Suzuki\,$^{2}$, Martin Voss\,$^{1,3,4}$  and Laura Kaltwasser\,$^{1}$ \\

\hspace{-0.5cm}{$^{1}$Berlin School of Mind and Brain, Humboldt-Universität zu Berlin, Germany
 \\
 $^{2}$ Sackler Centre for Consciousness Science, University of Sussex, Brighton BN1 9QJ, UK\\
$^{3}$ Department for Psychiatry and Psychotherapy, Charité University Medicine, Berlin, Germany\\
$^{4}$ St. Hedwig Krankenhaus, Berlin, Germany}\\





\subsection{Participants and Data}
XXX Participants were tested for 1 hour recording. 
Sitting at a table and not moving much (Allowed to watch a movie?) 
Counter-balancing the conditions if first assessed by Arduino and then medical device, sometimes other way around.


\section{Results}
Comparison Arduino vs. Medical device in terms of: \\
-Number of samples after 1 hour and size of datafile\\
-Heartbeats in total (assessed by a human)
-Sensitivity and specificity rates
-Delay of heartbeat detection
-Delay for sending to computer (Advantage of C++ since it has a directer machine layer?) 

\section{Conclusions}
Is this setup (Hardware and software) suitable to get reliable results?\\
Is the delay low enough to be considered to be used in studies where latency is important? E.g. VR-Study? \\
Giving access to everybody who wants to use it with the Code and easy to change Pins according to the Arduino/ Modules that will be of use and the hardware circuit

\section*{Author Contributions}
TM conceptualized and designed the study; The idea and first implementation of transferring the heartbeat into a VR-environment came from K.S.; T.M. wrote the code and assembled the device. TM acquired and analyzed the data under the supervision of MV and LK; TM wrote the manuscript; All authors contributed to manuscript revision, read and approved the submitted version.
